Anomalous Transport In Magnetized Shear Flow

After the initial stage of fast expanding of the hot Universe comes epoch of temperature fall and subsequent formation of dense clouds of hydrogen. Due to process of accretion some of this clouds became compact objects. Initially accretion is spherical, but then take the shape of the disk, and this 2D disk collect matter more efficient than 3D sphere. Accretion disks provide the mechanism of redistribution of angular moment and extraction of potential energy,leads to occurrence of compact objects from gas clouds. To fall moving along a spiral trajectory on the central gravitating body, a particle rotation around must reduce angular moment and energy. Outward of angular moment and movement of gas particles in the opposite direction (to the central body) happens due to of viscose friction. We can think that the disc is composed of multiple adjacent rings friction each other, each inner ring has a large angular velocity to the adjacent outer ring and thus friction of the drive ring decreased the rate of internal. The occurrence of intense dissipation in accretion flows is among the long-standing unsolved problems in astrophysics. Revealing how the magnetized turbulence creates shear stress tensor is of primary importance to understand the heating mechanism and the transport of angular momentum in accretion disks. The transport of angular momentum at greatly enhanced rates is important for the main problem of cosmogony, that is understanding the dynamics of creation of compact astrophysical objects. Without a theory explaining the enhanced energy dissipation in accretion flows of turbulent magnetized plasma we would have no clear picture of how our solar system has been created, why the angular momentum of the Sun is only 2% of the angular momentum of solar system, while carrying 99% of the solar system's mass.

==> src/src.tex <==
\appendix
\addappheadtotoc

\chapter{Source Code}

\begin{verbatim}
 ////////////////////////////////////////
// 
//  After the Fortran90 program by E. Penev published in
//  T. Mishonov and E. Penev
//  "Thermodynamics of Gaussian fluctuations and paraconductivity in 
//  layered superconductors"  International Journal of 
//  Modern Physics B, Vol. 14, No. 32 (2000) 3831-3879.
//  
//  Former C version of this program is given in the preprint:
//  T.M. Mishonov, S.I. Klenov, E.S. Penev,
//  "Temperature dependence of the specific heat and the penetration
//  depth of anisotropic-gap BCS superconductors for a factorizable
//  pairing potential"  http://arxiv.org/abs/cond-mat/0212491v5
//  [cond-mat.supr-con] [v5] Wed, 28 Apr 2004
//
//  Owners: Todor M. Mishonov & Zlatan D. Dimitrov 
// 
//  Description: 
//  Finds the limit of a series in the case where only
//  the first N+1 terms b[i] are known.
//
//  Method:
//  The routine operates by applying the epsilon-algorithm
//  to the sequence of partial sums of a series supplied on input.
//  For desciption of the algorithm, please see 
//  G. Baker, Jr., and P. Graves-Morris, Pad´ Approximants,
//  G.-C. Rota editor, 
//  Encyclopedia of Mathematics and its Applications, 
//  Vol. 13, (Addison-Wesley, London,1981), Table 3, p. 78; 
//  C. Brezinski, Pad´e-type Approximation and General  Orthogonal
//  Polynomials (Birkhauser, 1980);
//  P. Wynn, Math. Tables Aids Comput. 10, 91 (1956);
//  D. Shanks, J. Math. Phys. 34, 1 (1955).
//
//////////////////////////////////////////////////////////////////////////////

                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        #include <stdio.h>
#include <math.h>
#include <string.h>


//////////////////////////////////////////////////////////////////////////////
//////////    EPSILON ALGORITH    ////////////////////////////////////////////
//////////////////////////////////////////////////////////////////////////////
long double summa( int n, long double b[n], int *iP, int *kP, 
long double *p_err, long double *pLimes, int *p_OK,int *p_nk, int *p_ierr )
// a[i], i=0 ... n
// Routine for calculation of optimal Pade approximant of series
{
int mnz=2;// Maximal Number of Zeroes in a[i]
int nz=0; // current Number of Zero a[i] at the moment

int i=0,k, imax, kPade=0, iPade=0, ierr=7,nPade, iOK=0, ndz=0;
// Pade approximant aLimes[iPade/kPade] +/- err;
// err == empirical evaluation of the error << 1
long double bmax=0, s[n],t[n][n],ew,aLimes=0,err,eps=1,norma=0,temp,scale=0;
float epsf=1,fLimes;
char report[100];

int mdl=1;// (modul) number of unified terms
int nk=(n+1)/mdl-1;
long double a[nk];


for(k=0;k<=nk;k++){
   a[k]=0;
   for(i=0;i<mdl;i++) 
     {a[k]+=b[mdl*k+i];}
                  }
n=nk;


for(eps=1;eps+1>1;eps/=2) // double precision machine epsilon should be a global variable
epsf=sqrt(eps); // atifitial single precision

// PROTECTION

for(i=0;i<=n;i++) norma+=fabs(a[i]);
if(norma==0) {ierr=2; strcpy(report,"norma==0"); goto label;} // this line is "insgurance" against all terms to be == 0

if( fabs(a[0]) > fabs(a[n]) ) for(i=0;i<=n;i++) {for(temp=0,k=i;k>=0;temp+=a[k],s[i]=temp,k--);}
                         else for(s[0]=a[0],i=1;i<=n;i++) s[i]=s[i-1]+a[i]; // summation starts from smallest terms
// implicitely we suppose s[-1]=0; the s[0]=s[-1]+a[0];
// then a[i]=s[i]-s[i-1] for i=0,1,2,3, ... in Fortran program Limes the array s[i] is the imput variable

for(i=1;i<=n;i++)
{
if( a[i] != 0) { nz=0; if( 1/fabs(a[i])>bmax ) { 
bmax=1/fabs(a[i]); err=fabs(a[i]); iPade=i;aLimes=s[i];ierr=1;
strcpy(report,"Usual Taylor summation");
						}
		}
if( a[i] == 0 ) {nz++; if( nz == mnz ) {aLimes=s[i-mnz]; iPade=i-nz, err=0; ierr=3; 
                                        strcpy(report,"a[i]==0,..., a[i-mnz] ==0; polynom?; no need of epsilon summation");
                                        goto label;} 
                }
} // the series could be fastly covergent -- no need of epsilon algorith the label means exit the end of the routine

for(i=0;i<=mnz;i++) scale+=fabs(a[i]);
for(i=0;i<=n;i++){ if(fabs(a[i])>scale/eps) {n=i; break;} } // good working line

//printf("n=%i, ierr=%i  \n",n,ierr);
if(n<3) {ierr=5; strcpy(report,"n<3"); aLimes=s[n]; iPade=n; goto label;} // this line is an "insgurance" for small n
// all partial summs sould be "comparable" within mashibe epsilon; a new technolosical detail

// a lot of unnecessary details above!

// INITIALIZATION 
for(i=0;i<=n;t[0][i]=s[i],i++);// epsilon table
for(i=0;i<=n-1;i++)
{
if(a[i+1] != 0) {b[i]=1/a[i+1]; 
                 t[1][i]=b[i]; // epsilon table
                } 
else {b[i]=0; 
      t[1][i]=b[i]; // epsilon table
      ndz++; 
      ierr= 4; 
      strcpy(report,"if( a[i+1] == 0) then 1/0=0");}// should be harmless division by zero
}

// BEGINING OF EPSILON ALGORITH
// epsilon algorith beginning with 2nd row: (E-W)*(S-N) ==1;
imax=n-2;
for(k=2;k<=n+1;k++) // odd k means pade row s[i]; even k help row b[i]
	{       
	
	if(k%2==0) { for(i=0;i<=imax;i++) 
			{s[i]=s[i+1]; 
                         ew=b[i+1]-b[i];
			 if(ew !=0) s[i]+=1/ew; 
			 t[k][i]=s[i]; // epsilon table
			}
		   }
         
	if(k%2==1) { for(i=0;i<=imax;i++) 
			{b[i]=b[i+1]; 
		         ew=s[i+1]-s[i];
			 if(ew !=0) b[i]+=1/ew; 		
                         t[k][i]=b[i]; // epsilon table
                                                if ( bmax < fabs(b[i]) ) {
						bmax=fabs(b[i]); // maximal help row element criterion; the MAIN detail! 
						aLimes=s[i];
						kPade=(k-1)/2;
						iPade=i+kPade;
						err=1/bmax;
						ierr=0;	
						strcpy(report,"ierr=0;The regular work of epsilon algorith");
			 						  }

                        }
		   }

		imax--; 
	if(imax<0) break;
	}
label: nPade=iPade+kPade+1;// label for emrgency exit
if(err/norma<epsf) {fLimes= (float) aLimes; iOK=1;}
printf("norma>>>>%Le\n",norma);
puts(report);
printf("iPade=%i,kPade=%i,err=%Le,ndz=%i,nz=%i,i=%i,nPade=%i,n=%i\n",iPade,kPade,err,ndz,nz,i,nPade,n);
printf(">>>>>iOK=%i<<<<<\n",iOK);
*iP=iPade;
*kP=kPade;
*p_err=err;
*pLimes=aLimes;
*p_OK=iOK;
*p_nk=nk;
*p_ierr=ierr;
return aLimes;
}

////////////////////////////////////////////////////////////////////////////////////////////////////

////////////////////////////////////////////////////////////////////////////////////////////////////
// FUNCTION

long double function (long double x)
{
int n=51,iPade, *p=&iPade ; //n=7 min pri sdvoiavane(mdl=2) ili n=3 
int kPade,iOK,nk,ierr;
long double result, err,aLimes,sign;
long double a[99];
int i=0;
  
/////
long double v[100],suma=0;
//long double alpha=0,beta=-0.5,gamma=0,delta=-0.025,eta=0.275,az=0,buki=0,vedi=0;
////

//HeunC(alpha,beta,gamma,delta,eta;Z)

/*v[0]=1;
v[1]=(gamma - alpha + beta*(gamma-alpha+1) + 2*eta)/(2*(beta+1));
for(i=2;i<n+1;i++)
{
	m=i-1;
			az=delta + (alpha*0.5)*(m+m + beta + gamma);
			buki=m*(m+1+beta+gamma-alpha) + 0.5*(gamma+eta+eta-alpha+beta*(1-alpha+gamma));
			vedi=-(m+1)*(m+1+beta);
			v[i]=-(v[i-1]*buki + v[i-2]*az)/vedi;
}

*/
sign=1;
v[0]=0;
for(i=1;i<=n;i++)
{
v[i]=sign/i;
sign=-sign;
//printf("v[%i]=%Lg\n",i,v[i]);
}

long double xn;
xn=1;
for(i=0;i<=n;i++)
{
a[i]=v[i]*xn;xn*=x;
//printf("a[%i]=%Lg\n",i,a[i]);
suma+=a[i];
}
//printf("\n suma= %.12Lf\n ",suma);
// ln(1+x)=x-x^2/2+x^3/3-x^4/4+x^5/5-...


/*
// here cut %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
int mdl=2;// number of unified terms
int nk=n/mdl;
for(k=0;k<=nk;k++){
   b[k]=0;
   for(i=0;i<mdl;i++) 
     {b[k]+=a[mdl*k+i];}
                  }
// here cut %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
*/

result=summa(n,a,p,&kPade,&err,&aLimes,&iOK,&nk,&ierr);
//printf("\n>>>>iPade=%i;kPade=%i;err=%Lg;aLimes=%Lg,iOK=%i\n",iPade,kPade,err,aLimes,iOK);
//printf("P[%i/%i]=%Lg  +/-  %Lg,      OK=%i, n=%i, ierr=%i\n",iPade,kPade,aLimes,err,iOK,nk,ierr);
return result;

}



int main(void)
{
long double x,z;

x=exp(1)-1;
//for(x=0.1;x<15;x+=0.1)
//{
z=function(x);//z=ln(e)=1;
printf("%Lg %.12Lf\n",x,z);
printf("ln(1+x)=%.12f\n",log(M_E));
//}

return 0;
}


\end{verbatim}


